Calabi-Yau techniques for Namikawa-Weyl groups

The field of symplectic singularities aims to build a 21st century Lie theory. A key development is the Namikawa-Weyl group, which generalizes the classical Weyl group of Lie algebras. Another cornerstone is the integration of categorical Calabi-Yau techniques, capturing the rich algebraic structure of these singularities. In this paper, we develop a systematic strategy to determine Namikawa-Weyl groups for representation spaces of Calabi-Yau-2 algebras, leveraging local-to-global functors, symmetry analysis, and $ A_{\infty} $-methods. Applying this approach to quiver varieties, we carry out the detailed calculations and recover Yaochen Wu's result.

==> app_excfiber/action.tex <==

\begin{itemize}
\item $ θ' $ is generic, or
\item $ (Q', α') $ is $ A_3 $, $ σ $ swaps two pairs of vertices, and $ θ' $ is nonzero, or
\item $ (Q', α') $ is $ D_4 $, $ σ $ involves all four outer vertices [i.e. but not two pairs], and $ θ' $ is nonzero.
\end{itemize}

